Learning Inconsistent Preferences with Gaussian Processes

We revisit widely used preferential Gaussian processes by Chu et al.(2005) and challenge their modelling assumption that imposes rankability of data items via latent utility function values. We propose a generalisation of pgp which can capture more expressive latent preferential structures in the data and thus be used to model inconsistent preferences, i.e. where transitivity is violated, or to discover clusters of comparable items via spectral decomposition of the learned preference functions. We also consider the properties of associated covariance kernel functions and its reproducing kernel Hilbert Space (RKHS), giving a simple construction that satisfies universality in the space of preference functions. Finally, we provide an extensive set of numerical experiments on simulated and real-world datasets showcasing the competitiveness of our proposed method with state-of-the-art. Our experimental findings support the conjecture that violations of rankability are ubiquitous in real-world preferential data.

==> content/LiteratureReview.tex <==
\section{Preferential Modelling}




\paragraph{Preferential learning with skew-symmetric constraints using data augmentation} 

%It is also worth mentioning that learning with skew-symmetric constraint is related to a larger problem known as learning with invariances. In particular, Van et al. \cite{van2018learning} proposed a kernel to model strictly invariant functions $f_{inv}$:
%\begin{equation}
%    k_{f_{inv}}(x, x') = \sum_{x_a \in A(x)} \sum_{x'_a \in A(x')} k(x_a, x_a') 
%\end{equation}
%where $A(x) := \{t(x)| t \in G\}$ and $G$ is the set of all invariant transformations that $f_{inv}$ respects, i.e. $f_{inv}(t(x)) = f_{inv}(t'(x))$ for all $t,t' \in G$. At first sight this kernel resembles our proposed skew-symmetric kernel (introduce later in eq (\ref{eq: sskernel})) but they are different. While $k_{f_{inv}}$ imposes invariant constraints on the arguments (i.e $ f_{inv}(t(x)) = f_{inv}(t'(x))$, we impose the (skew-symmetric) constraint directly on the function itself instead (i.e $g(x, x') = -g(x', x)$).

\paragraph{Recovering latent structures in preferential data}





%Another latent structure of interest is the \textit{Rankability} of duelling data. The concept of Rankability is first introduced by Anderson et al.\cite{anderson2019rankability}, which measures the dataset's inherent ability to produce a meaningful ranking of its items. The authors proposed \textsc{edge-r}, a rankability measure that is based on an integer program for computing the minimum number of edge changes made to a directed graph in order to obtain a complete dominance graph i.e. an acyclic tournament graph. Recently Cameron et al. \cite{cameron2020graph} proposed \textsc{spec-r}, a more scalable rankability score that utilise the spectral-degree characterisation of complete dominance graphs instead. In our work, we will consider a third probabilistic characterisation of rankability, \textsc{bayes-r}, by conducting a Bayesian hypothesis test between \textsc{pref-gp} and our proposed \textsc{generalised pref-gp}.

